Process matrices on generalised theories

We extend the process-matrix framework for defining indefinite causal orders to a broad class of generalised physical theories. We give a simple re-axiomatisation of spacetime contexts in terms of naturality over classical probes, which precisely captures non-contextual assignment together with compatibility with convexity and coarse-graining within local laboratories. Using this compositional perspective, we give a clean characterisation of theories in which abstract spacetime contexts admit a process-matrix representation, and we pin down the precise conditions (satisfied by classical theory, quantum theory, and a Boxworld-like theory) under which the supermap and process-matrix perspectives on higher-order processes coincide.

==> figs/giant.tex <==
\begin{tikzcd}[ampersand replacement=\&]
  \& F(a\otimes b)^* \otimes Fa \otimes Fb \ar[d,"\cong"] \ar[dl,"\cong"'] \ar[r,"1\otimes l"] \& F(a\otimes b)^* \otimes F(a\otimes b) \ar[d,"\cong"] \ar[dr,"l"] \ar[r,"s^{-1}\otimes 1"] \&  (F(a\otimes b))^* \otimes F(a\otimes b) \ar[r,"\varepsilon"] \& i_\parr \ar[dddddddd,equal]\\
  F(a\otimes b)^* \otimes Fa \otimes (Fb^*)^* \ar[d,"\cong"'] \ar[r,"1\otimes 1\otimes s"] \& F(a\otimes b)^* \otimes Fa \otimes Fb^{**} \ar[d,"\cong"] \ar[r,"1\otimes l"] \& F(a\otimes b)^* \otimes F(a\otimes b^{**}) \ar[d,"\cong"] \& |[yshift=-1.8em,overlay]| F((a\otimes b)^*\otimes (a\otimes b)) \ar[ddl,"\cong"] \ar[ddddddl,"F\epsilon"] \& \\
  F(a^*\parr b^*) \otimes Fa \otimes (Fb^*)^* \ar[d,"l\otimes 1"'] \ar[r,"1\otimes 1\otimes s"] \& F(a^*\parr b^*) \otimes Fa \otimes Fb^{**} \ar[d,"l\otimes 1"] \ar[r,"1\otimes l"] \& F(a^*\parr b^*) \otimes F(a \otimes b^{**}) \ar[d,"l"] \& \& \\
  F((a^*\parr b^*)\otimes a) \otimes (Fb^*)^* \ar[d,"F\delta\otimes 1"'] \ar[r,"1\otimes s"] \& F((a^*\parr b^*)\otimes a) \otimes Fb^{**} \ar[d,"F\delta\otimes 1"] \ar[r,"l"] \& F((a^*\parr b^*)\otimes a \otimes b^{**}) \ar[d,"F(\delta\otimes 1)"] \& \& \\
  F((a^*\otimes a)\parr b^*) \otimes (Fb^*)^* \ar[d,"F(\varepsilon\parr 1)\otimes 1"'] \ar[r,"1\otimes s"] \& F((a^*\otimes a)\parr b^*) \otimes Fb^{**} \ar[d,"F(\varepsilon\parr 1)\otimes 1"] \ar[r,"l"] \& F(((a^*\otimes a)\parr b^*) \otimes b^{**}) \ar[ddl,"F((\varepsilon\parr 1)\otimes 1)"] \& \& \\
  Fb^* \otimes (Fb^*)^* \ar[dddr,"\varepsilon"'] \ar[r,"1\otimes s"] \& Fb^* \otimes Fb^{**} \ar[d,"l"] \& \& \& \\
  \& F(b^*\otimes b^{**}) \ar[d,"F\varepsilon"] \& \& \& \\
  \& F(i_\parr) \ar[d] \& F(i_\parr) \ar[l,equal] \& \& \\
  \& i_\parr \& \& \& i_\parr \ar[lll,equal]
\end{tikzcd}

